Categorical Probabilistic Theories

We present a simple categorical framework for the treatment of probabilistic theories, with the aim of reconciling the fields of Categorical Quantum Mechanics (CQM) and Operational Probabilistic Theories (OPTs). In recent years, both CQM and OPTs have found successful application to a number of areas in quantum foundations and information theory: they present many similarities, both in spirit and in formalism, but they remain separated by a number of subtle yet important differences. We attempt to bridge this gap, by adopting a minimal number of operationally motivated axioms which provide clean categorical foundations, in the style of CQM, for the treatment of the problems that OPTs are concerned with.

==> eptcsdata.tex <==
\providecommand{\firstpage}{367}
\providecommand{\publicationstatus}{Bob Coecke and Aleks Kissinger (Eds.):\\ 14th International Conference on Quantum Physics and Logic (QPL)\\
EPTCS 266, 2018, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.266.23}{10.4204/EPTCS.266.23}}
\pdfoutput=1

